From Text to Insight: Large Language Models for Materials Science Data Extraction

The vast majority of materials science knowledge exists in unstructured natural language, yet structured data is crucial for innovative and systematic materials design. Traditionally, the field has relied on manual curation and partial automation for data extraction for specific use cases. The advent of large language models (LLMs) represents a significant shift, potentially enabling efficient extraction of structured, actionable data from unstructured text by non-experts. While applying LLMs to materials science data extraction presents unique challenges, domain knowledge offers opportunities to guide and validate LLM outputs. This review provides a comprehensive overview of LLM-based structured data extraction in materials science, synthesizing current knowledge and outlining future directions. We address the lack of standardized guidelines and present frameworks for leveraging the synergy between LLMs and materials science expertise. This work serves as a foundational resource for researchers aiming to harness LLMs for data-driven materials research. The insights presented here could significantly enhance how researchers across disciplines access and utilize scientific information, potentially accelerating the development of novel materials for critical societal needs.

==> old_text.tex <==

% \begin{itemize}
%     \item Key questions: How do we get from what we mined to something we can put into a model? What is to consider here? (Can we provide a decision tree?) 
%     \item It goes beyond just getting the text
%     \begin{itemize}
%         \item correct analysis might require an understanding of the layout (see discussion here \url{https://arxiv.org/abs/2309.10952})
%         \item Ordering of blocks if you have multiple blocks. Text blocks must be placed into the right reading order 
%     \end{itemize}
%     \item However, images are still treated separately in the reasoning steps (requires vision model) 
%     \item When should we use OCR and a text model, and when should we go directly for a multimodal model? What are pros and cons?
%     \item Tools: 
%     \begin{itemize}
%         \item Nougat
%         \item Marker 
%         \item doctor
%         \item unstructured
%         \item Classical: Tesseract, GROBID, PDFMiner, Cermine, ParsCit
%         \item check what Jacqui Cole does in PDFDataExtractor\autocite{Zhu_2022}:
%         \begin{itemize}
%             \item They use PDFMiner
%             \item They have hard-coded rules for parsing the layout
%         \end{itemize}
%     \end{itemize}
%     \item Document cleaning
%     \begin{itemize}
%         \item There are many things one maybe does not need: 
%         \begin{itemize}
%             \item References
%             \item Authors 
%             \item Page numbers (page heading/footers)
%             \item Table and figure captions if those are not included 
%             \item Acknowledgements
%         \end{itemize}
%     \end{itemize}
% \end{itemize}


% \begin{itemize}
%     \item \textbf{General model performance}: the first step is always to try how general big \glspl{llm} works with different prompts techniques. If the vocabulary of the field is not very specific, a general model may return really good results in terms of accuracy and recall avoiding the need of further pre-training or fine-tuning saving a lot of time and effort.
%     \item \textbf{Cost}: it is important to consider how big is the extraction corpus, and once considered that see if it is possible to assume the costs associated to the closed-source \glspl{api} models.
%     \item \textbf{Latency}: if the application needs for a faster response from the model, then probably it is better to use an open-source model that can be working locally instead of waiting for the closed-source \gls{api} responses.
%     \item \textbf{Specificity of the Task}: when the task is very specific or complex, a fine-tuning step should be consider to improve the model in that task.
%     \item \textbf{Data type}: if the data to extract is private or may contain sensitive personal information such as medical information, then probably the best option is to use an open-source model that works locally.\autocite{tang2023does}
%     \item \textbf{Computational resources and expertise}: before taking the decision of pre-training or fine-tuning a model, it must be consider that these learning paradigms are highly computational costly and need of some expertise to correctly apply them.
%     \item \textbf{Time constrains}: since pre-training and fine-tuning need of high computational resources, they also take more time that can go from some days to some weeks depending of the model size and the amount of data.
%     \item \textbf{Availability of labeled data}: a full pre-training need a lot of tokens, i.e. some billions of tokens are needed to pre-train BERT models. Fine-tuning needs less data and could work really good with some hundreds of corrected labeled data, but more than 1000 labeled examples would be the ideal number.
% \end{itemize}
%     \begin{itemize}
%         \item How well it works a general model with different prompt techniques? Good → Step 2, bad →step 3
%         \item Can you assume the costs associated with the API? Yes → Decision: General model with prompt techniques, No → Step 4
%         \item Do you have the computational resources and expertise needed for pre-train and fine-tune your own model? Yes → Step 4 No → Step 8
%         \item Is the data highly specific? Yes → Step 5 No → Step 6
%         \item Pre-train a model and test it on a sample database. Is the performance adequate? Yes→ Decision: pre-trained model, No → Step 6
%         \item Do you have enough high-quality labeled data for fine-tuning? Yes → Decision: Fine-tuned model No→ Step 7
%         \item Is it feasible to obtain more high-quality labeled data needed for fine-tuning? Yes → Decision Fine-tuned model, No → Step 8
%         \item Reconsider using a general model. Try more shots which are representative of the entire corpus of data. → Step 1
%     \end{itemize}


% Should we learn from context, not at all, or by changing model weights?
% \begin{itemize}
%     \item Key question: How do we decide what modeling paradigm we use? What different approaches are there and what are the tradeoffs? \url{https://twitter.com/karpathy/status/1655994367033884672}
%     \item Good tracker of what model probably can do what \url{https://docs.llamaindex.ai/en/stable/module_guides/models/llms/#llm-compatibility-tracking}
%     \begin{itemize}
%         \item Test the waters of your use case through: Zero-Shot Prompting
%         \item Explore what’s already possible if you collect a bit of data to demonstrate the behavior you are looking for: Few-Shot Prompting
%         \item If Few-Shot Prompting is not cutting it, you can look into actually changing the model itself by providing it [prompt, response] samples: Supervised Fine-Tuning
%     \end{itemize}
%     \item What are key factors we need to take into account to make this decision? 
%     \begin{itemize}
%         \item Specificity of the Task / How general does the approach need to be? 
%         \item Availability of Training Data
%         \item Computational Resources and Expertise
%         \item Time Constraints
%         \item Baseline Model Performance
%     \end{itemize}
%     \item Based on the points above, a decision tree that GPT-4 recommends (we should edit it, but it is a good starting point): 
%     \begin{enumerate}
%         \item Assess Task Specificity: Is the data highly specific or does it use specialized terminology?:  Yes → Proceed to Step 2. No → Go to Step 5.
%         \item   Evaluate Baseline Model Performance:  Test the pre-trained model on a sample dataset. Is the performance adequate? Yes → Go to Step 5. No → Proceed to Step 3. 
%         \item   Check Availability and Quality of Training Data. Do you have sufficient high-quality, labeled data for fine-tuning? Yes → Proceed to Step 4. No → Consider improving or acquiring more data. If not feasible, go to Step 5.
%         \item Review Resources and Expertise. Do you have the computational resources and technical expertise needed for fine-tuning? Yes → Proceed to fine-tune the model. No → Consider outsourcing or acquiring resources. If not feasible, go to Step 5.
%         \item  Final Decision. Based on the above evaluations, decide: Use the pre-trained model as is if it meets the necessary performance levels and constraints. Opt for fine-tuning if the model’s current performance is inadequate, and you have the resources to carry out the process effectively.
%     \end{enumerate}
%     \item Prompting is a science of its own:
%     \begin{itemize}
%         \item There is a lot of folk knowledgde, such as \enquote{tipping} the model \url{https://minimaxir.com/2024/02/chatgpt-tips-analysis/}
%         \item There is huge risk for data leakage. People do not really report how they tuned their prompts and they typically only have one eval set. However, one very fundamental concept of statistcial learning is that we want to only use the test set for testing. Validation should happen on a validation set. 
%         \item \url{https://openreview.net/forum?id=oRKWhmtUG6}
%         \item \url{https://jina-ai-gmbh.ghost.io/content/files//2024/04/DSPy-Not-Your-Average-Prompt-Engineering--1-.pdf}
%         \item There is some folk knowledge that an \enquote{unsure} option can improve things
%     \end{itemize}
%     \item General vs. specifically pretrained model \url{https://pubs.acs.org/doi/10.1021/acs.jcim.4c00063}
%     \item How do we decide if we finetune the model or not? \url{https://hamel.dev/blog/posts/fine_tuning_valuable.html}
%     \item A bit related \textcite{balaguer2024rag}
%     \item Many examples use few-shot prompting 
%     \begin{itemize}
%         \item \url{https://twitter.com/goodside/status/1564437905497628674}
%         \item \url{https://twitter.com/eugeneyan/status/1636366239873515521}
%         \item there are also various prompt-chaining approaches, e.g. \url{https://doi.org/10.48550/arXiv.2307.12701}
%         \item Multiple query prompting (rephrasing the prompt to get more robust results)
%     \end{itemize}
% \end{itemize}

% \paragraph{Frontiers/Foundation model programming}
% \begin{itemize}
%     \item While current approaches mostly work on hard-coded prompt templates and utilizing only one technique, there is a growing number of tools that allow to autonomously optimize the part between input and output in the form of pipelines, for example, by automatically tuning prompts 
%     \begin{itemize}
%         \item \enquote{We argue that this approach, while pervasive, can be brittle and unscalable—conceptually akin to hand-tuning the weights for a classifier.} \textcite{khattab2023dspy}
%         \item use signatures as the main interface
%         \item compilation means that you use a teacher LM or some data you have 
%     \end{itemize}
%     \item then there is, in principle, no different between prompting and fine-tuning as the compiler will just care about input/output pairs (you just need to swap out what they call \enquote{Teleprompter})
% \end{itemize}


% LLMs have a finite context window. Hence, we cannot provide the model with unlimited text (e.g., 2048 tokens for GPT-4). We can only provide subsets, such as parts of a paper. This raises the natural question of how to select the subsets.

% \begin{itemize}
%     \item Key questions: How do we deal with the finite context length of LLM and resources that might be larger than the context length? What are tradeoffs one can make? How do we decide what to use? 
%     \item A very important thing we need to state there is that in our scientific setting, we often rely on being able to refer across a long paper because a compound might be discussed in different ways in different parts of a paper
%     \item The fact that chunking is super important is also reflected in OpenAI's recent RAG updates \url{https://x.com/GregKamradt/status/1780668006705828245} (but OpenAI makes it work without semantic chunking \url{https://x.com/athyuttamre/status/1780684020449202408})
%     \item Important use case for RAG: you have a giant corpus (companies) and you want to extract text from that. Running it all completely through GPT-4 will cost a lot. Embedding first and only retrieving the relevant chunks is something that is way more reasonable.
%     \item Vector store needed?
%         \begin{itemize}
%             \item Either you chunk or do retrieval on the fly \url{https://x.com/jerryjliu0/status/1709343094582452634?s=20}
%         \end{itemize}
%     \item Various chunking approaches: 
%         \begin{itemize}
%             \item Fixed number of tokens: Best for scenarios where the text does not have complex dependencies that span across large sections. It's simple and easy to implement. 
%             \item Semantic chunking: This method uses natural divisions in the text, such as paragraphs, sections, or sentences, to guide chunking. It relies on understanding the structure of the document to make more meaningful divisions. There is some link (in spirit) to TextTiling \textcite{hearst1997text}
%             \item Recursive chunking: Split recursively upon separators. Langchain's RecursiveCharacterTextSplitter class splits text using default separators (note that even that is not straightforward as punctuation might be used in very different ways)  %(“\n\n”, “\n”, “ “,””) 
%         \end{itemize}
%         They can be used overlapping and non-overlapping. They can be implemented with simple rule-based approaches, models or hybrids of models and rules
%     \item What happens in a multimodal case? 
%     \item Chunking considerations: \url{https://www.pinecone.io/learn/chunking-strategies/}
%     \item here they just look at chunking \url{https://arxiv.org/html/2402.05131v2}
%     \item See also some of the thinking in auto-merging retrieval \url{https://freedium.cfd/https://generativeai.pub/advanced-rag-retrieval-strategies-auto-merging-retrieval-dc3f869654c4} (if a bunch of nearby context chunks are retrieved, merge them into one bigger “chunk” so the LLM has a holistic view of the larger document.)
%     \item Tools like NLTK can be used to split text into sentences. This ensures that chunks don’t break sentences. However, splitting by paragrams can be more meaningful as paragraphs typically represent distinct ideas.
%     \item It can be useful to have overlap between chunks:
%     \begin{itemize}
%         \item context preservation (surrounding text needed to understand passage)
%         \item smoothing transition
%     \end{itemize}
%     \item More advanced is semantic splitting, which splits text at semantically meaningful points. For example, ChunkBert: \url{https://arxiv.org/abs/2310.20558}
%     \item there might already be a classification step that decides if relevant information is in there or not (e.g. in \url{https://arxiv.org/abs/2302.04914})
%     \item Visualization \url{https://chunkviz.up.railway.app/} and article \url{https://www.rungalileo.io/blog/mastering-rag-advanced-chunking-techniques-for-llm-applications#chunk-attribution} (they have some discussion about how to evaluate chunking effectiveness) 
%     \item Some inspiration for the notebook here \url{https://github.com/FullStackRetrieval-com/RetrievalTutorials/blob/main/tutorials/LevelsOfTextSplitting/5_Levels_Of_Text_Splitting.ipynb}
%     \item Techniques such as infinite attention might minimize the need for chunking \textcite{munkhdalai2024leave} (see also the table there). Relevant techniques Transformer-XL, Longformer
%     \item In some sense, the need for chunking is the full motivation behind RAG, see a nice discussion here \url{https://blog.normalcomputing.ai/posts/2023-09-12-supersizing-transformers/supersizing-transformers.html} (the technique they propose there has some links to Infiniattention) and this is quite related to \textcite{wu2022memorizing} (i.e., you let attention access a vectorstore [non differentiable] with previous sequences)
% \end{itemize}

%Some users used few-shot prompting to do the binary classification of text fragments, determining whether they contain suitable data for extraction.\cite{Zheng_2023, Choi2024} 


% \begin{itemize}
%     \item \url{https://faktion.com/blog/guided-text-generation-with-large-language-models/}
%     \item work of Bob West (EPFL) 
%     \item what are pros and cons of using constrained decoding? 
%     \item which of the following techniques are most promising, which should I use? 
%     \item very basic (just prompting) example of using Pydantic/JSON schema \url{https://xebia.com/blog/enforce-and-validate-llm-output-with-pydantic/}
%     \item \url{https://www.llmparser.com/}
%     \begin{itemize}
%         \item Prompts to generate a certain schema
%         \item Prompts to return confidence
%     \end{itemize} 
%     \item JSONformer: Generate one field at a time and only sample from a subset of tokens. JSONFormer fills in the fixed, repetitive schema tokens and allows the LLM to only generate the variable content tokens
%     \item Guidance \url{https://github.com/guidance-ai/guidance}
%     \item OpenAI function calling \url{https://gist.github.com/kylemcdonald/dbac21de2d7855633689f5526225154c}
%     \item Guardrails \url{https://docs.guardrailsai.com/} Guardrails is a tool designed to enforce the structure of text extraction tasks by validating LLM outputs against a defined Pydantic schema. Users can wrap LLM API calls to validate, structure, and correct outputs by initializing a Guard object with the output schema. See examples here \url{https://txt.cohere.com/validating-llm-outputs/}
%     \item \url{https://github.com/stanfordnlp/dspy}
%     \item \url{https://zenodo.org/records/10020588}
%     \item Work by Chris Mungall:
%     \begin{itemize}
%         \item SPIRES  employs zero-shot learning capabilities of LLMs to interpret prompts and return information that aligns with a user-defined schema. It recursively performs prompt interrogation against an LLM, obtaining responses that match the provided schema and using existing ontologies to provide identifiers for matched elements
%         \begin{itemize}
%             \item \url{https://arxiv.org/abs/2304.02711} 
%             \item \url{https://www.youtube.com/watch?v=z38lI6WyBsY}
%             \item \url{https://github.com/monarch-initiative/ontogpt}
%         \end{itemize}
%         \item see also \url{https://berkeleybop.github.io/project/AI/} for an overview 
%     \end{itemize}
%     \item \url{https://ar5iv.labs.arxiv.org/html/2306.08302}
%     \item using black-box models (without access to logit distribution) \url{https://ar5iv.labs.arxiv.org/html/2401.09967v1}
%     \item DOMINO \url{https://arxiv.org/abs/2403.06988} enforcing constraints in a subword-aligned manner, leveraging pre-computation and speculative decoding.
%     \item Grammar constrained decoding \url{https://ar5iv.labs.arxiv.org/html/2305.13971}
%     \item \url{https://ar5iv.labs.arxiv.org/html/2305.13917}
%     \item Interesting discussion here via finite state machines \url{https://blog.normalcomputing.ai/posts/2023-07-27-regex-guided-generation/regex-guided-generation.html} for the \url{https://github.com/outlines-dev/outlines/tree/main} library. Nice anecdotes 
%     \begin{itemize}
%         \item \enquote{The Manhattan project of our time, AutoGPT, has an issue label dedicated to incorrect JSON outputs.}
%         \item see the paper \url{https://arxiv.org/abs/2307.09702}
%     \end{itemize}
% \end{itemize}

% \subsection{Grounding}

==> sections/applications.tex <==
\section{Application example}
See Notion resources list:

%\begin{itemize}
    %\item High entropy alloys, and critical cooling rates of metallic glasses. bulk modulus dataset to demonstrate with hand-curated data for evals. Material - property - unit extraction. Zero-shot. \textcite{Polak_2024}
%ChatExtract: conversational LLM and prompt engineering, a set of engineered prompts applied to a conversational LLM with follow-up questions, databases for critical cooling rates of metallic glasses and yield strengths of high entropy alloys are developed, prompt engineering proposed to extract Material, Value, Unit triplet

    %\item \textcite{buehler2024accelerating}
    %\begin{itemize}
    %    \item They also use Nougat
    %    \item They generate knowledge graphs using LLamaindex, i.e, using one-shot prompting
    %\end{itemize}
%\end{itemize}    

    %\item \textcite{Luu_2023} conversational large language model finetuned using LoRA, RAG is used using Llama Index, use of Nougat OCR

    %\item Ceder Nat Comm %\textcite{dagdelen_structured_2024}, Ceder's old stuff
% fine-tuned LLM for performing joint named entity recognition and relation extraction (NERRE)

    %\textcite{Kononova_2019} generated a dataset of “codified recipes” for solid-state synthesis automatically extracted from scientific publications
    and a bunch of applications from their team
     
    %\textcite{Lee_2024_oxidation} This work introduced an automated data-extraction pipeline involving a CNN for table detection and an LLM for the selective extraction of scientific data on experimentally-measured oxidation potentials of organic molecules.
    
    \item Digital Discovery has multiple articles by now
    
    %\item See also reaction data extraction \url{https://github.com/qai222/LLM_organic_synthesis} (currently in review) with nice explorer \url{https://qai222.github.io/LLM_organic_synthesis/}. Preprint \textcite{Ai_2024}. This also gives nice examples of the limitations of a fine-tuned model: It might fail to generalize on new types of unstructured input. They also nicely show where conventional techniques fail (e.g. with reference tokens)    
    
    %\item Luc Patiny and Guillaume Godin \textcite{patiny_automatic_2023} explores extracting analytical experiment results from literature solely through prompt engineering. While this method can extract structured data by including in-prompt data schema, it relies on closed-source LLMs and performs poorly when numerical values are involved. Based on their analysis, the remaining major issue was molecule name parsing.
    
    \item Yaghi for MOFs, also multimodal:
    \begin{itemize}
        \item their first paper
    \begin{itemize}
        \item In \textcite{Zheng_2023} they use a multistep workflow: They first classify which sections likely contain synthesis information and then extract data one-by-one
        \item All based on prompts (also the request for structured output) 
        \item For classification into sythesis/non-synthesis paragraphs they used few-shot prompting (in the SI they compare zero-shot with few-shot) 
        \item They use-embeddings for prefiltering (perhaps an example for Sherjeel to discuss). Their Figure 3 is actually decent and something we could do ourselves using an open model (notebook on GitHub) 
        \item They use \enquote{interactive prompt refinement}, i.e., ask ChatGPT to refine the prompt
        \item They also use ChatGPT for entity resolution (i.e. to expand abbreviations) 
        \item They claim that they manually extracted the ground truth for more than 800 compounds (that is a good eval set --- and way more effort than we have put into it ;)) 
    \end{itemize}
    
    \item in their second paper they use GPT-4-V \textcite{Zheng_2024} --> example for the multimodal chapter   
    \begin{itemize}
        \item namely nitrogen isotherms, PXRD patterns, TGA curves, crystal structure or topology illustrations, and other gas sorption isotherms
        \item manually labeled more than 6.2K images (one image is one page of a paper)  for presence of the different spectra
        \item also focus on extracting data from nitrogen adsorption isotherms. But there they do not extract precise values but rather let the model classify the saturation regime
        \item They mention (but do not use) DSpy for prompt optimization \textcite{khattab2023dspy}
    \end{itemize}

    %\item Hoex for solar cells, fine-tuning \textcite{xie_creation_2024} Creation of a structured solar cell material dataset and performance prediction using large language models, A new NLP task called structured information inference (SII) was introduced, which involves advanced capabilities such as computational analysis and component inference together with RE.
    
    %\item Samuel J. Cooper et al. Finding and analyzing micrographs in preprint \textcite{lei_materials_2024}
   
    \item Antunes et al. Crystal structure generation (CIF). \textcite{antunes_crystal_2024} trained a LLM specifically designed for crystal generation on an extensive corpus of textual representations of inorganic crystal structures, specifically in the Crystallographic Information File (CIF) format, instead of relying solely on natural language corpora, or chemical compositions alone. The model is directly trained on the standardized and tokenized text contents of the CIF files.
    
    %\item Construction of functional materials knowledge graph. Extracting triples from papers. \textcite{ye_construction_2024}
    
    %\item Sparks et al. Extracting JSON form materials papers (Gemini Pro). Mentions the problem of not having a good way to evaluate the JSON output. \textcite{Sayeed_2024} 

    %\item Action sequence extraction for organic synthesis 
    \begin{itemize}
        %\item IBM \textcite{Vaucher_2020}
        %\item Cronin SynthReader \textcite{Mehr_2020} rule-based natural language processing (NLP) algorithm called SynthReader specialized to extract sequences of processes from synthesis descriptions
    \end{itemize}
    
    \item Companies: 
    \begin{itemize}
        \item \url{https://www.data-revival.com/} / \url{https://www.linkedin.com/company/data-revival-ltd/about/}, slides \autocite{munday_2024_10808354} (not clear though if they use LLMs, but they certainly could use V-LLM).
        The University of Southampton’s chemistry department: utilised AI-driven natural language processing techniques, as well as chemical structure recognition, to extract all the types of chemical information required to create a useful, searchable database from Chemistry Lab Notebooks
        %conversion of chemical structures into SMILES/INCHI
        \item Bayer \url{https://www.linkedin.com/posts/gressling_i-am-excited-to-share-my-upcoming-talk-activity-7175400607011237889-VFiT?utm_source=share&utm_medium=member_desktop} 
    \end{itemize}
    
    %\item \textcite{Thway_2024} These authors noted that the LLM fails to extract information from a paragraph that requires human intuition. However, the answer becomes more consistent when they provide appropriate examples in the prompt. They also found that extracting information sequentially one by one with standard answers gives the best results. They include formatting checks in the prompt as additional questions to improve performance.
    
    %\item \textcite{Lee_2024_synthesis} utilized a hybrid approach mixing search-based algorithms and fine-tuning of a LLM for NERRE to extract multi-sourced seed-mediated gold nanoparticle (AuNP) synthesis recipes from the literature. Using regular expression (regex) to avoid issues with confusing or overlapping acronyms
    
\end{itemize}

Perhaps also integrate into the sections above as it fits (this separate section might be a bit awkward). 


%- M. Zaki, N. A. Krishnan, et al., Extracting processing and testing parameters from materials science literature for improved property prediction of glasses, Chem. Eng. Process-Process Intensif., 2022, 180, 108607 extract synthesis, processing and testing conditions, of oxide glasses to study hardness of glasses, spaCy's NER tool for text, the OCR and data extraction tool WebPlotDigitizer to extract from graphs\textcite{Zaki2022}


%- V. Venugopal, S. Sahoo, M. Zaki, M. Agarwal, N. N. Gosvami and N. A. Krishnan, Looking through glass: Knowledge discovery from materials science literature using natural language processing, Patterns, 2021, 2(7), 100290. knowledge extraction from inorganic glasses’ literature, ChemDataExtractor for extraction of chemical species, latent Dirichlet allocation (LDA) (An unsupervised NLP algorithm to classify abstracts and search semantically linked publications, caption cluster plot (CCP) to summary of images and plots\textcite{Venugopal2021} To automate image comprehension, in this domain, \textcite{Venugopal2021} propose the caption cluster plot (CCP) \gls{nlp} technique to group the information contained in all the figure captions in the corpus by their semantic similarity.

